Stored energies for electric and magnetic current densities

Electric and magnetic current densities are an essential part of electromagnetic theory. The goal of the present paper is to define and investigate stored energies that are valid for structures that can support both electric and magnetic current densities. Stored energies normalized with the dissipated power give us the Q factor, or antenna Q, for the structure. Lower bounds of the Q factor provide information about the available bandwidth for passive antennas that can be realized in the structure. The definition that we propose is valid beyond the leading order small antenna limit. Our starting point is the energy density with subtracted far-field form which we obtain an explicit and numerically attractive current density representation. This representation gives us the insight to propose a coordinate independent stored energy. Furthermore, we find here that lower bounds on antenna Q for structures with e.g. electric dipole radiation can be formulated as convex optimization problems. We determine lower bounds on both open and closed surfaces that support electric and magnetic current densities. The here derived representation of stored energies has in its electrical small limit an associated Q factor that agrees with known small antenna bounds. These stored energies have similarities to earlier efforts to define stored energies. However, one of the advantages with this method is the above mentioned formulation as convex optimization problems, which makes it easy to predict lower bounds for antennas of arbitrary shapes. The present formulation also gives us insight into the components that contribute to Chu's lower bound for spherical shapes. We utilize scalar and vector potentials to obtain a compact direct derivation of these stored energies. Examples and comparisons end the paper.

==> macro.tex <==
\newcommand{\Hil}{\set{H}}

% general macros

% text macros
\newcommand{\cf}{{\it cf.\/}\ }
\newcommand{\etal}{{\it et.\/ al.\/}, }
\newcommand{\ie}{{\it i.e.\/}, }
\newcommand{\eg}{{\it e.g.\/}, }
\newcommand{\sind}[1]{{\text{{\tiny $#1$}}}}

% font macros

\newcommand{\symb}[1]{\boldsymbol{#1}}%\mbox{\boldmath $#1$}}
\newcommand{\set}[1]{\mathrm{#1}}
\newcommand{\fat}[1]{\mbox{\boldmath $#1$}}
\newcommand{\sfat}[1]{{\mbox{\scriptsize \boldmath $#1$}}}

% math symbols

\newcommand{\RR}{\mathbb{R}}

\newcommand{\bone}{\mathchoice {\rm 1\mskip-4mu l} {\rm 1\mskip-4mu l}
{\rm 1\mskip-4.5mu l} {\rm 1\mskip-5mu l}}
\newcommand{\LL}{\mathcal{L}}
\newcommand{\KK}{\mathcal{K}}
\newcommand{\CC}{\mathcal{C}}
\newcommand{\iu}{\mathrm{i}}
\newcommand{\ju}{\mathrm{j}}
\newcommand{\grad}{\nabla}
\newcommand{\Laplace}{\Delta}
\renewcommand{\exp}[1]{\mathrm{e}^{#1}}
\newcommand{\lexp}[1]{\mathrm{e}^{#1}}
%\DeclareMathOperator{\sbj}{\mathrm{\j}}
%\DeclareMathSymbol{\jj}{\mathalpha}{letters}{"10}
%\newcommand{\jj}{\text{\j}}
\newcommand{\sbj}[1]{\mathop{}\!\j_{#1}}
\newcommand{\shd}{\mathrm{h}^{(2)}}



\newcommand{\RE}{\mathop{\set{Re}}}
\newcommand{\IM}{\mathop{\set{Im}}}
\newcommand{\supp}{\mathop{\mathrm{supp}} }
\newcommand{\domain}[1]{\set{D}( #1 )}
\newcommand{\Range}[1]{\set{R}( #1 )}
\newcommand{\Null}[1]{\set{N}( #1 )}
\newcommand{\closure}[1]{\left\{ #1 \right\}_{\mathrm{cl}} }
\newcommand{\adj}{*}
\newcommand{\adjoint}[1]{#1^{\adj}}
\newcommand{\conj}[1]{\bar{#1}}
\newcommand{\commute}[2]{[#1,#2]}
\newcommand{\Res}[2]{\mathrm{Res}\left\{ #1; #2 \right\}}
%\newcommand{\diff}{\mathop{\mathrm{\mathstrut{d}}}\!}%Diff op.
\newcommand{\diff}{\mathop{}\!\mathrm{d}}%Diff op.
\newcommand{\DF}{\mathcal{D}}
\newcommand{\Span}{\mathop{\mathrm{span}}}
\newcommand{\Oh}{\mathcal{O}}
%\newcommand{\deg}{\mathop{\mathrm{deg}}}
%\newcommand{\arg}{\mathop{\mathrm{arg}}}
\newcommand{\diag}{\mathop{\mathrm{diag}} }

\newcommand{\Div}{\nabla\cdot}
\newcommand{\Rot}{\nabla\times}


% spaces
\newcommand{\Hone}{\set{H}^1}
\newcommand{\Honeloc}{\Hone_{\mathrm{loc}}}
\newcommand{\pspace}{\Gamma_{c}}
\newcommand{\Rpspace}{\Gamma_{r}}
\newcommand{\TM}{\set{T}_{\vsol}\Rpspace}
%\newcommand{\Space}{\Gamma}
\newcommand{\MS}{\TM}
\newcommand{\MSL}{\set{T}_{\sol}\pspace}
\newcommand{\CMS}{\Hone(\mathbb{R}^2,\mathbb{C}^2)}
\newcommand{\LCS}{\Ltwo(\mathbb{R}^2,\mathbb{C}^2)}
\newcommand{\Yspace}{\set{Y}}
\newcommand{\Htwo}{\set{H}^2}
\newcommand{\Sob}[1]{\set{H}^{#1}}
\newcommand{\C}[1]{\set{C}^{#1}}
\newcommand{\Ltwo}{\set{L}^2}
\newcommand{\Lp}[1]{\set{L}^{#1}}
\newcommand{\dotp}[2]{\langle #1,#2\rangle}
\newcommand{\dote}[2]{\dotp{#1}{#2}_{0}}
\newcommand{\nrme}[1]{\|#1\|_0}       % chi supp
\newcommand{\nrm}[1]{\|#1\|}       % chi supp
\newcommand{\Cdot}[2]{\dotp{#1}{#2}_{\Ltwo(\mathbb{R}^2,\mathbb{C}^2)}}
\newcommand{\Rdot}[2]{\dotp{#1}{#2}_{\Ltwo(\mathbb{R}^2)}}
\newcommand{\Cnorm}[1]{\|#1\|_{\Ltwo(\mathbb{R}^2,\mathbb{C}^2)}}
\newcommand{\Rnorm}[1]{\|#1\|_{\Ltwo(\mathbb{R}^2)}}

% theorems & etc.
\newtheorem{prop}{Proposition}
\newtheorem{lem}{Lemma}
\newtheorem{rem}{Remark}
\newtheorem{que}{Question}
\newtheorem{thm}{Theorem}
%\newtheorem{cor}{Corollary}[thm]
\newtheorem{cor}{Corollary}
\newtheorem{ass}{Assumption}[thm]
\newtheorem{work}{Exercise}
\newtheorem{hint}{Hint}[work]
\newtheorem{Def}{Definition}


% local macros

\newcommand{\GG}{G(\vr,\vr';k)}
\newcommand{\Gp}{G^+(\vr,\vr';k)}
\newcommand{\Gpm}{G^\pm(\vr,\vr';k)}
\newcommand{\Gn}{G^-(\vr,\vr';k)}

%constants
\newcommand{\eps}{\varepsilon}

% sources
\newcommand{\va}{\boldsymbol{a}}
\newcommand{\vu}{\boldsymbol{u}}
\newcommand{\vb}{\boldsymbol{b}}
\newcommand{\vc}{\boldsymbol{c}}
%\newcommand{\vd}{\boldsymbol{d}}
\newcommand{\hc}{\hat{\boldsymbol{c}}}
\newcommand{\vK}{\boldsymbol{K}}
\newcommand{\vJ}{\boldsymbol{J}}
\newcommand{\vA}{\boldsymbol{A}}
\newcommand{\vB}{\boldsymbol{B}}
\newcommand{\vF}{\boldsymbol{F}}
\newcommand{\vT}{\boldsymbol{T}}
\newcommand{\vM}{\boldsymbol{M}}
\newcommand{\vL}{\boldsymbol{L}}
\newcommand{\vX}{\boldsymbol{X}}
\newcommand{\vrho}{\boldsymbol{\rho}}

%distances & directions
\newcommand{\ve}{\boldsymbol{e}}
\newcommand{\vh}{\boldsymbol{h}}
\newcommand{\vr}{\boldsymbol{r}}
\newcommand{\vR}{\boldsymbol{R}}
\newcommand{\ha}{\hat{\boldsymbol{a}}}
\newcommand{\he}{\hat{\boldsymbol{e}}}
\newcommand{\hx}{\hat{\boldsymbol{x}}}
\newcommand{\hy}{\hat{\boldsymbol{y}}}
\newcommand{\hz}{\hat{\boldsymbol{z}}}
\newcommand{\hk}{\hat{\boldsymbol{k}}}
\newcommand{\hn}{\hat{\boldsymbol{n}}}
\newcommand{\hr}{\hat{\boldsymbol{r}}}
\newcommand{\hth}{\hat{\boldsymbol{\theta}}}
\newcommand{\hphi}{\hat{\boldsymbol{\varphi}}}
\newcommand{\hrho}{\hat{\boldsymbol{\rho}}}
\newcommand{\hnu}{\hat{\boldsymbol{\nu}}}
\newcommand{\hnz}{\hat{\boldsymbol{\nu}}_0(\vr')}
\newcommand{\nnz}{\hat{\boldsymbol{\nu}}_0}
\newcommand{\vxi}{\boldsymbol{\xi}}

% fields
\newcommand{\vE}{\boldsymbol{E}}
\newcommand{\vH}{\boldsymbol{H}}
\newcommand{\vD}{\boldsymbol{D}}

\newcommand{\Ys}{\boldsymbol{Y}_{\sigma m \ell}}
\newcommand{\vY}{\boldsymbol{Y}}
\newcommand{\vYo}{\boldsymbol{Y}_{1\sigma m \ell}}
\newcommand{\vYt}{\boldsymbol{Y}_{2\sigma m \ell}}
\newcommand{\vYd}{\boldsymbol{Y}_{3\sigma m \ell}}
\newcommand{\Yoo}{\boldsymbol{Y}_{1\sigma m \ell,1}}
\newcommand{\Yto}{\boldsymbol{Y}_{2\sigma m \ell,1}}
\newcommand{\Yot}{\boldsymbol{Y}_{1\sigma m \ell,2}}
\newcommand{\Ytt}{\boldsymbol{Y}_{2\sigma m \ell,2}}
\newcommand{\Yo}{\boldsymbol{Y}_{1e01}}
\newcommand{\Yt}{\boldsymbol{Y}_{2e01}}


\newcommand{\vG}{\boldsymbol{G}}
\newcommand{\Wec}{W_{\mrm{e,c}}}
\newcommand{\Wmc}{W_{\mrm{m,c}}}
\newcommand{\Wet}{W_{\mrm{e}}}
\newcommand{\We}{W_{\mrm{e,F}}}
\newcommand{\Wem}{W_{\mrm{em}}}
\newcommand{\Wmt}{W_{\mrm{m}}}
\newcommand{\Wm}{W_{\mrm{m,F}}}
\newcommand{\rP}{P_{\mrm{rad}}}
\newcommand{\tP}{P_{\mrm{tot}}}
\newcommand{\lP}{P_{\mrm{abs}}}

\newcommand{\tR}{\tilde{R}}

